Online Visual Analytics of Text Streams

We present an online visual analytics approach to helping users explore and understand hierarchical topic evolution in high-volume text streams. The key idea behind this approach is to identify representative topics in incoming documents and align them with the existing representative topics that they immediately follow (in time). To this end, we learn a set of streaming tree cuts from topic trees based on user-selected focus nodes. A dynamic Bayesian network model has been developed to derive the tree cuts in the incoming topic trees to balance the fitness of each tree cut and the smoothness between adjacent tree cuts. By connecting the corresponding topics at different times, we are able to provide an overview of the evolving hierarchical topics. A sedimentation-based visualization has been designed to enable the interactive analysis of streaming text data from global patterns to local details. We evaluated our method on real-world datasets and the results are generally favorable.

==> application.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Potential Applications}\label{sec:application}

We deployed the system as an internal desktop application within Microsoft. A panel of experts, including customer relationship managers, public relations managers, and researchers, systematically evaluated and investigated the potential applications of the system.  Several highly promising applications were identified.

%We invited several experts, including 3 customer relationship managers, 3 public relations managers, and 4 researchers, to systematically evaluate and discuss the potential usage of the system.


First, our system can be employed in customer relationship management to help analysts fully understand customer-related information on social media.
A variety of social media outlets enable customers to communicate with each other more easily and take a more active role as market players~\cite{Hennig2010}.
%Since the buzz of the crowd on social media provides a great deal of information that
%was not available before, businesses have started leveraging social media to profile customers, derive brand perception, understand buying trends, and improve customer satisfaction.
The implication for businesses is obvious: they need to understand what customers are saying about them in various social media outlets.
For this reason, customer relationship managers are very interested in using the system to quickly understand customers' comments and feedbacks on social media.
For example, a customer relationship manager utilized the system to analyze customer feedback related to ``Xbox'' on Twitter and blogs.
He appreciated the topic hierarchies provided by the system, which enabled him to immediately identify overall patterns as well as directly interact with the visualization to examine the finer-grained topics.
He commented, ``This is very helpful in finding something unexpected.''

Second, public relations managers claimed that the system can help them better analyze company-related information, such as news, blogs, and microblogs.
For example, a Microsoft public relations analyst wants to analyze a number of important events related to the company that occurred in the first half of 2013.
These events are the announcement of the new Xbox, Motorola suing the company, and the release of Windows 8.
To analyze these events, the public relations analyst employed the system to examine the Microsoft-related news stream and understand the major topics and how they have changed over time.
With the system, the analyst could better understand how these events are related to one another at different granularities and their impact over time.
Furthermore, he can determine whether the company's public relations strategies have succeeded (e.g., the amount of the excitement generated by the product release).

Finally, researchers utilized our system to study major research topics in their fields as well as the splitting/merging relationships among the topics of interest over time.
With this toolkit, they easily identified the research topics and related publications that match their research interest.
Interestingly, a sociology PhD student found that he could use the system to study the media framing effects in a news corpus.
He was intrigued when he found that a sub-topic changed its parent between two adjacent trees.
In his exploration, the sub-topic exemplified by the keywords ``Windows, Kinect" changed its parent from ``Windows" to ``Xbox."
He said, ``Parent topics provide the context for the sub-topics.
A concrete sub-topic such as ``Kinect'' can be mentioned in the context of ``Windows'' in the first week, and in the context of ``Xbox'' in the next week.
This defines different perspectives or ways of communicating about topics.
This phenomenon is widely studied in our field and is referred to as \textbf{media framing}.
I believe this system can definitely help detect such framing phenomena." 

==> data.tex <==
% !TEX root = EvoTree-KDD.tex


\section{Evolutionary Tree Clustering}\label{sec:data}
%In this section, we briefly introduce evolutionary multi-branch tree clustering~\cite{Wang2013}, which is used to extract a sequence of multi-branch topic trees \{${T^t}$\} from text streams.
\kg{This section briefly introduces} evolutionary multi-branch tree clustering~\cite{Wang2013}, which is used to extract a sequence of multi-branch topic trees \{${T^t}$\} from text streams.
%To describe the quality of \{${T^t}$\}, two important measures, fitness and smoothness, are employed~\cite{Wang2013}.
Two important measures, \kg{namely,} fitness and smoothness, are employed~\cite{Wang2013} to describe the quality of \{${T^t}$\}.
%The fitness of a tree $T^t$ measures how well the documents at time $t$ are organized.
The fitness of a tree $T^t$ measures how well the documents are organized at time $t$.
%On the other hand, the smoothness ensures the structural similarity between $T^t$ and $T^{t-1}$, if the document content does not deviate much from $t-1$ to $t$.
\kg{Smoothness} ensures the structural similarity between $T^t$ and $T^{t-1}$ if document content does not deviate much from $t-1$ to $t$.
Wang et al.~\cite{Wang2013} formulated the fitness and smoothness in a Bayesian online filtering process \kg{as follows}:
%\dup{To capture both fitness and tree structure changes in the data, we formulated the learning procedure as a Bayesian online filtering process in our previous work~\cite{Wang2013}:}
\begin{equation}\label{eq:learningframework}
\small
\begin{split}
&p(T^t | \mathcal{D}^t, T^{t-1})  \propto  p(\mathcal{D}^t | T^t) p(T^t | T^{t-1}).  \\
%& = \frac{p(\mathcal{D}_m^t|T_m^t)}{p(\mathcal{D}_i^t|T_i^t)p(\mathcal{D}_j^t|T_j^t)} \cdot  \frac{1}{Z} \exp\Big(-\lambda V_{T^{t-1}}(\{T_i^t,T_j^t\} \rightarrow T_m^t)\Big).
\end{split}
\end{equation}
%The first term corresponds to the likelihood ratio of the original BRT algorithm~\cite{Blundell2010} (fitness), and the second term is the smoothness cost.
The first term corresponds to the likelihood ratio of the original BRT algorithm~\cite{Blundell2010} (fitness), whereas the second term \kg{denotes} the smoothness cost.
%This recursive objective function can be solved with a dynamic programming algorithm.
%With this formulation, the new tree $T^t$ depends on the likelihood of the current data $p(\mathcal{D}^t | T^t)$ and the conditional prior $p(T^t | T^{t-1})$ that measures the difference between $T^t$ and $T^{t-1}$.
\kg{Based on} this formulation, the new tree $T^t$ depends on the likelihood of the current data $p(\mathcal{D}^t | T^t)$ and the conditional prior $p(T^t | T^{t-1})$ that measures the difference between $T^t$ and $T^{t-1}$.

%In additional to \textbf{\normalsize a sequence of coherent topic trees \{${T^t}$\}}, the evolutionary tree model also outputs the following two types of information:
In \kg{addition} to \textbf{\normalsize a sequence of coherent topic trees \{${T^t}$\}}, the evolutionary tree model also outputs the following types of information:

\begin{compactitem}
%\item \dup{A sequence of evolving \textbf{topic trees}, where an interior node of a topic tree is a topic and a leaf node is a document.
%In postprocessing, the documents that directly belong to an interior node also form a topic whose parent is the interior node.}
%With this processing, each document is a leaf node.
%\vspace{1mm}
%\item \textbf{\normalsize Topic pairs:} For any adjacent topic trees $T^i$ and $T^{i+1}$, our model maps the related topics together to generate a set of topic pairs. Intuitively, the relations are induced from their document content or the splitting/merging operations taken during the tree generation process.
\item \textbf{\normalsize Topic pairs:} For any adjacent topic trees $T^i$ and $T^{i+1}$, our model maps the related topics \kg{collectively} to generate a set of topic pairs. \kg{The} relations are \kg{intuitively} induced from their document content or \kg{from} splitting/merging operations \kg{performed} during the tree generation process.
%\dup{For two adjacent topic trees, the clustering model maps the related topics, such as similar topics and topics with a splitting/merging relationship, together.}
%\dup{We call two mapped topics a topic pair.}
%\vspace{1mm}
%\item \textbf{\normalsize Document pairs:} For each topic pair between $T^i$ and $T^{i+1}$, our model also maps similar documents together to generate a set of document pairs.
\item \textbf{\normalsize Document pairs:} For each topic pair between $T^i$ and $T^{i+1}$, our model also maps similar documents \kg{collectively} to generate a set of document pairs.
\end{compactitem}


%%\subsection{Clustering Results}
%\dup{Given a text stream, evolutionary tree clustering generates the following outputs.} %\looseness=-1
%
%\begin{compactitem}
%\item \dup{A sequence of evolving \textbf{topic trees}, where an interior node of a topic tree is a topic and a leaf node is a document.
%In postprocessing, the documents that directly belong to an interior node also form a topic whose parent is the interior node.}
%With this processing, each document is a leaf node.
%%\vspace{1mm}
%\item \dup{A set of \textbf{topic pairs} between two adjacent topic trees.}
%\dup{For two adjacent topic trees, the clustering model maps the related topics, such as similar topics and topics with a splitting/merging relationship, together.}
%\dup{We call two mapped topics a topic pair.}
%%\vspace{1mm}
%\item \dup{A group of \textbf{document pairs} within each topic pair. The model also maps two similar documents together, each of which is from each of the topic pairs. These documents are referred to as a document pair.}
%\end{compactitem}


==> discussion.tex <==
\section{Discussion}

==> evaluation_b.tex <==
\section{Evaluation}\label{sec:evaluation}

In this section, a quantitative evaluation of the proposed evolutionary tree cut algorithm is conducted.
The usefulness of our approach is then demonstrated with a case study.



\input{quantative_b.tex}

\subsection{Case Study}
This section highlights how \emph{RoseRiver} helps analyze large text streams by applying it to a news dataset, Obama data.
444,432 news articles that contain the keyword ``Obama,'' were collected from Sep. 1, 2012 to Jan. 14, 2013.
Grouped by week, the articles were organized into 18 topic trees. %(Fig.~\ref{fig:obamatree}).
%The average number of the first level nodes is 41, and the tree depth is 5($\pm 1$).
The tree depths varied from 4 to 5, the total node numbers changed from 144 to 297, and the node
number of the first level ranged from 18 to 79.
%\begin{figure}[ht]
%  \centering
%  \includegraphics[width=\columnwidth]{fig/obamatree}
%  \caption{Example topic tree for Obama data.}
%  \label{fig:obamatree}
%\end{figure}


To provide an overview of the news data to users, our system automatically extracted several initial focus nodes that can suitably represent the dataset and are distinct from one another.
In our implementation, a clustering method, the mean-shift algorithm, was utilized to cluster the topic at the first level because it is the most abstract level and can represent the topic tree very well.
Four clusters were detected in the Obama data.
For each cluster, we selected the node closest to the cluster center as a focus node.
Four focus nodes were automatically derived to generate the default overview (Fig.~\ref{fig:obama}(a)).
In the overview, the four colors represent four different topics: ``Iran'' (red), ``Tax'' (yellow), ``Debate'' (green), and ``Gun Control'' (purple).
As shown in Fig.~\ref{fig:obama}(a), significant variations existed; however, some overall patterns clearly stood out.
The green and yellow topics were dominant and divided the entire time period into two parts.
The red topic was small but persistent and the purple one was large but irruptive.

In the first half of the time period (before Nov. 3), the ``Debate'' (green) topic dominated and unsurprisingly ended in the week of Nov. 6, 2012, the date when Obama was reelected as president.
In addition, the ``Tax'' (yellow) topic was partially related to the ``Debate'' (green) topic from time to time.
Initially, the yellowish green topic (marked as \textbf{A} in Fig.~\ref{fig:obama}(a)), a mixed topic of ``Debate'' and ``Tax,'' merged with the green one.
This merging was caused by the tax-related debates (``Obama, Romney Clash on Economy, Taxes in First Debate'').
The yellowish green topic gradually split from the green one because its focus shifted to the economy, jobs, and the fiscal cliff.
If users are interested in tracking the mixed topic, they could interactively split the topic nodes and extract them from the green topic (Fig.~\ref{fig:obama}(b)).


Similarly, the ``Iran'' (red) topic  interacted with the ``Debate'' (green) topic in the week of Oct. 20 (marked as \textbf{B} in Fig.~\ref{fig:obama}(a)).
After splitting the topic nodes into small ones (Fig.~\ref{fig:obama}(c)), a red topic node that contained several news articles on ``Iran'' was observed
For example, one of the articles had the title ``Obama, Romney on Israel and Iran.'' This article clearly indicates why these two topics merged.

After the week of Nov. 3 (the second half of the time period), the ``Tax'' (yellow) topic dominated the view.
Considering that it has fewer connections with other topics, it was more isolated than the ``Debate'' topic.
Within these topics, the yellow nodes were almost fully connected with one another; thus, the ``Tax'' was also a relatively stable topic.

Although the ``Tax'' (yellow) topic was dominant during this time period, two greenish nodes (marked as \textbf{C} and \textbf{D} in Fig.~\ref{fig:obama}(a)) still appeared.
Clearly, these two topics have different evolution patterns.
Judging from the connections between \textbf{C} and the other nodes, \textbf{C} was likely a momentary topic.
To verify this hypothesis, we examined \textbf{C}'s content and found that it was focused on ``Romney blames loss on Obama's `gifts' to voters,'' which was indeed a momentary event.
On the other hand, \textbf{D} was fully connected to the yellow nodes. This connection indicates \textbf{D} contains news articles related to both the ``Debate'' and ``Tax'' topics. For example, one of the articles had the title ``GOP fights President Barack Obama on his campaign promise to raise taxes on the rich.''\looseness=-1


The ``Gun Control'' (purple) topic, which was caused by the Connecticut Elementary School massacre on Dec. 14, 2012, was then explored.
The event caused a topic burst in the week of Dec. 15.
Its horizontal offset indicates that it is a high-level topic node.
%Although the topic has a burst in the week of December 15, our system still finds several related topics, colored in purple, before the burst (marked as dotted rectangles in Fig.~\ref{fig:obama}(a)).
%Since they are highly related to our focus node, they are still successfully separated from the others.
%For example, in the week of Dec. 1, 2012 (marked as \textbf{E}), a node of only five documents talks about ``Obama to Push Gun Control in Second Term?''.
Then we split the big purple node and checked the two smaller topics in it (Fig.~\ref{fig:obama}(d)).
The lower node was mainly about the public discussion on gun control.
The strong connection of this node to the topic on the right indicates that it was still the major topic at the next time point.
When the node was split further, more detailed topics revealed themselves (Fig.~\ref{fig:obama}(e)).
From top to bottom, these topics were ``NRA calls for armed guards at every school,'' ``Obama turns to Biden on gun control measures,'' ``Guns fly off shelves,'' ``Assault weapons ban,'' and ``Connecticut school shooting: how to talk to your kids'' (marked as \textbf{F} to \textbf{J}, respectively).
The upper node, which represents follow-up news to the tragedy, has weaker connections to the right.
This condition indicates that the topic shrunk considerably at the next time point.

\begin{figure}[t]
  \vspace{-2mm}
  \centering
  \includegraphics[width=\columnwidth]{fig/clintonoverview}
  \vspace{-5mm}
  \caption{``Bill Clinton'' related topics.}
  \label{fig:clintonoverview}

\end{figure}
%  \vspace{-4mm}

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{fig/2clintonoverview}
    \vspace{-3mm}
  \caption{Topics related to ``Bill Clinton'' and ``Hillary Clinton.''\looseness=-1}
  \vspace{-3mm}
  \label{fig:2clintonoverview}
\end{figure}

%from Shixia, the below story can be deleted if the qualitative evaluation need more space.



The search function can help users explore more specific topics.
For example, we entered ``Bill Clinton'' in the search box.
The first topic node recommended by our system is about the speech at the Democratic National Convention on Sep. 5, 2012.
We selected it as the focus node and visualized the result.
As shown in Fig.~\ref{fig:clintonoverview}, the topic was only active in the first week (marked as \textbf{A}).
However, in the week of Oct. 20, a small but highly related topic node appeared (marked as \textbf{B}).
We clicked it to see the detailed content and found that it contained two sub-topic nodes: ``Bill Clinton to rally for Obama at Springs Preserve'' and ``Hillary Clinton says she's `unlikely' to stay Secretary of State'' (marked as \textbf{C}).
To further explore these nodes, we regarded both nodes as new focus nodes and transformed the visualization.
Fig.~\ref{fig:2clintonoverview} shows that the two Clintons mainly have one overlapping topic (marked as \textbf{D}), which is ``Bill Clinton's DNC speech: Setting the stage for Hillary in 2016?''

%In the middle of Fig.~\ref{fig:2clintonoverview}, our tree cut algorithm successfully splits the context topic and reveals two small relevant topics hidden inside, which are a discussion about ``Poll: Clinton favored in 2016 in Iowa''.

The topics on Hillary Clinton in the top of Fig.~\ref{fig:2clintonoverview} can be  divided into two parts (marked by \textbf{F} and \textbf{G}).
\textbf{F} is about the Libya Attack, in which Hillary Clinton was highly involved.
In the week of Oct. 13, the article with the title ``Hillary Clinton Takes Blame for Benghazi Attack'' ended that topic (marked by \textbf{E}).
\textbf{G} contains two separate topics related to Hillary Clinton whose colors indicate that one is more relevant to the focus than the other.
In fact, the greener one is about Hillary Clinton herself.
For example, two articles have the titles ``Clinton is the people's choice for 2016 Prez bid: Poll,'' and ``Obama calls Clinton to wish her well as she recovers from concussion.''
However, the other is about the secretary of state candidates, in which Hillary Clinton is partially involved.





==> overview.tex <==
\begin{figure*}[ht]
  \centering

  \includegraphics[width=\linewidth]{fig/overview}
  \caption{System pipeline: (a) generate evolving topic trees (dotted lines represent matched topics between times); (b) generate evolving tree cuts (the star is the user-selected focus node); (c) reorganize the topics according to the Degree-of-Interest (DOI) values; (d) align topic nodes by their depths; (e) color and scale topic nodes by the DOI values; (f) extract matched documents for the matched topics; (g) generate the final visualization.}\looseness=-1
  \label{fig:overview}
  \vspace{-3mm}
\end{figure*}

\section{Problem Formulation}
Fig.~\ref{fig:overview} briefly illustrates our system pipeline.
The input is a set of documents with time stamps.
First, we extract a sequence of topic trees from the input documents by our evolutionary tree clustering technique, which aims to better organize the topics at different times, as well as match correlated topics between adjacent topic trees.
Second, we transform tree clustering results into a set of salient topics that can well represent the large clustering results and be effectively visualized.
A user selects one or more topics of interest as the focus node(s).
Based on the focus node(s), the tree cut algorithm extracts a set of representative topics for each tree.
The algorithm also makes the representative topic sets at different times coherent with each other.
However, the cut algorithm may still extract too many topics that cannot be clearly displayed on the limited display area.
To tackle this, a mean-shift clustering algorithm~\cite{comaniciu2002mean} is employed to further group the extracted topics.
Meanwhile, the matched documents within the matched topics are extracted based on the relationships between the topics selected by our tree cut algorithm.
Finally, the transformed results, including the topics nodes on each tree cut, matched topics and documents, are visualized for further exploration and analysis.
